Learning to Condition: A Neural Heuristic for Scalable MPE Inference

We introduce learning to condition (L2C), a scalable, data-driven framework for accelerating Most Probable Explanation (MPE) inference in Probabilistic Graphical Models (PGMs), a fundamentally intractable problem. L2C trains a neural network to score variable-value assignments based on their utility for conditioning, given observed evidence. To facilitate supervised learning, we develop a scalable data generation pipeline that extracts training signals from the search traces of existing MPE solvers. The trained network serves as a heuristic that integrates with search algorithms, acting as a conditioning strategy prior to exact inference or as a branching and node selection policy within branch-and-bound solvers. We evaluate L2C on challenging MPE queries involving high-treewidth PGMs. Experiments show that our learned heuristic significantly reduces the search space while maintaining or improving solution quality over state-of-the-art methods.

==> algorithms/beam_search_algo.tex <==
\begin{wrapfigure}[20]{r}{0.5\textwidth} 
\vspace{-10pt} % tweak vertical space if needed
\begin{algorithm}[H]
\DontPrintSemicolon
\KwIn{PGM $\mathcal{M}$, Scoring Function $\mathcal{F}$, Evidence $\mathbf{E}$, Time Limit $tl$, Maximum Decisions $\mathcal{D}_{max}$, Beam Width $W$}
\KwOut{MPE Solution}
Initialize beam $B \gets [(0, \mathbf{E})]$ \; % (score, updated evidence)

\For{$d = 1$ to $\mathcal{D}_{max}$}{
    Initialize candidate list $C \gets []$\;
    \ForEach{$(s, E_{updated})$ in $B$}{
        \ForEach{variable-value pair $(X, x)$}{
            $E_{new} \gets E_{updated} \cup (X = x)$\;
            $s_{new} \gets \mathcal{F}(E_{new})$\;
            $(s_{new}, E_{new})$ to $C$\;
        }
    }
    $B \gets$ Sort $C$ by $s$ and retain top $W$ sequences\;
}

$(s_{best}, \mathbf{E_{best}}) \gets \text{TopCandidate}(B)$\;
$\text{rec} \gets \texttt{SolveMPE}(\mathcal{M}, \mathbf{E_{best}}, tl)$\;
\Return $\text{rec}$
\caption{Beam Search for Conditioning}\label{alg:beam_search}
\end{algorithm}
\vspace{-10pt} % tweak to control space below the figure
\end{wrapfigure}

==> algorithms/data_collection.tex <==
\begin{wrapfigure}[28]{r}{0.55\textwidth} % r for right side, 0.55 width (adjust as needed)
\vspace{-12pt} % tweak vertical space if needed
\begin{algorithm}[H]
\DontPrintSemicolon

\KwIn{PGM $\mathcal{M}$, Query Ratio $qr$, Dataset Type $dt$, Max Depth $d_{max}$, Max Choices $c_{max}$}
\KwOut{Dataset $DB$}

\textbf{Function} \texttt{SolveMPE}($\mathcal{M}, \mathbf{E}, \mathbf{e}$): \\
\Indp
    Run MPE solver on $\mathcal{M}$ with $\mathbf{E} = \mathbf{e}$\;
    \Return $\{ \text{time}, \text{\#nodes}, \text{assign} \}$ \\
\Indm

\textbf{Function} \texttt{Sample}($\mathbf{S}, n$): \\
\Indp
    \Return Randomly selected $n$ elements from $\mathbf{S}$\;
\Indm

$\mathbf{X} = \mathbf{x} \leftarrow \text{Sample generated from } \mathcal{M}$ \;
$\mathbf{Q} \gets \texttt{Sample}(\mathcal{V}, qr \cdot |\mathcal{V}|)$ \; 
$\mathbf{E} \gets \mathcal{V} \setminus \mathbf{Q}$ \tr{define $\mathcal{V}$}\;
%$d \gets \texttt{Sample}(\{0, 1, \dots, d_{max}\}, 1)$  \;

%$\mathbf{Q_d} \gets \texttt{Sample}(\mathbf{Q}, d)$ \;
%$\mathbf{E} \gets \mathbf{E} \cup \mathbf{Q_d}, \quad \mathbf{Q} \gets \mathbf{Q} \setminus \mathbf{Q_d}$ \;

$\text{rec} \gets \texttt{SolveMPE}(\mathcal{M}, \mathbf{E}, \mathbf{x}_{\mathbf{E}})$ \;

\If{$dt = \text{ranking}$}{
    $\text{opt} \gets \text{rec}[\text{assign}]$ \;
    $\mathbf{C} \gets \texttt{Sample}(\mathbf{Q}, c_{max})$ \;
    
    \For{each $C \in \mathbf{C}$}{
        $c \gets \text{opt}[C]$ \;
        $\mathbf{E}^{'} \gets \mathbf{E}, \quad \mathbf{e}^{'} \gets \mathbf{e}$ \;
        $\mathbf{E}^{'} \gets \mathbf{E}^{'} \cup \{C\}, \quad \mathbf{e}^{'} \gets \mathbf{e}^{'} \cup \{c\}$\;
        $\text{rec} \gets \texttt{SolveMPE}(\mathcal{M}, \mathbf{E}^{'}, \mathbf{e}^{'})$
    }
}

\text Store in DB

\caption{Data Collection for Training Neural Network for Conditioning}\label{algo:dataset}
\end{algorithm}
\vspace{-10pt} % tweak to control space below the figure
\end{wrapfigure}

==> fig_tex_files/decimation_scip3.tex <==
\begin{figure}[htbp]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/supplement/win-comparison3.pdf}
    \label{fig:win-comparison3}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/supplement/win-comparison5.pdf}
    \label{fig:win-comparison5}
  \end{subfigure}
  \caption{Neural vs. baseline methods for beam search with width value set to 3 (SCIP oracle). (a) Win counts; (b) Log-likelihood gaps. Color: Darker green = stronger, darker red = weaker performance. Grey: Timeouts (30s).}
  \label{fig:combined-wins}
\end{figure}

\FloatBarrier

% \begin{wrapfigure}[47]{r}{0.275\linewidth}
%     \vspace{-10pt} % Adjust as needed to align with surrounding text
%     \centering
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/supplement/win-comparison3.pdf}
%         \caption{Wins vs. oracle by time limit for all methods (SB: Full Strong Branching, LO: \textsc{L2C-OPT}, LR: \textsc{L2C-Rank}).}
%         \label{fig:win-comparison3}
%     \end{subfigure}
%     \vspace{1em}
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/supplement/ovno-ranking-gap3.pdf}
%         \caption{\textsc{L2C-Rank} vs. oracle $\mathcal{LL}$ gap by $\mathcal{D}_{max}$ (cols) and graphical model (rows).}
%         \label{fig:ovno-ranking-gap3}
%     \end{subfigure}
%     \vspace{-15pt}
%     \caption{Neural vs. baseline methods for beam search with width value set to 3 (SCIP oracle). (a) Win counts; (b) Log-likelihood gaps. Color: Darker green = stronger, darker red = weaker performance. Grey: Timeouts (30s).}
%     \label{fig:combined-gap3}
% \end{wrapfigure}


==> fig_tex_files/decimation_scip5.tex <==
\begin{figure}[htbp]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/supplement/ovno-ranking-gap3.pdf}
    \label{fig:ovno-with-ranking-gap3}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/supplement/ovno-ranking-gap5.pdf}
    \label{fig:ovno-with-ranking-gap5}
  \end{subfigure}
  \caption{Neural vs. baseline methods for beam search with width value set to 3 (SCIP oracle). (a) Win counts; (b) Log-likelihood gaps. Color: Darker green = stronger, darker red = weaker performance. Grey: Timeouts (30s).}
  \label{fig:combined-ovno-with-ranking-gap}
\end{figure}

\FloatBarrier
% \begin{wrapfigure}[47]{r}{0.275\linewidth}
%     \vspace{-10pt} % Adjust as needed to align with surrounding text
%     \centering
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/supplement/win-comparison5.pdf}
%         \caption{Wins vs. oracle by time limit for all methods (G: Graph, SB: Full Strong Branching, LO: \textsc{L2C-OPT}, LR: \textsc{L2C-Rank}).}
%         \label{fig:win-comparison5}
%     \end{subfigure}
%     \vspace{1em}
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/supplement/ovno-ranking-gap5.pdf}
%         \caption{\textsc{L2C-Rank} vs. oracle $\mathcal{LL}$ gap by $\mathcal{D}_{max}$ (cols) and graphical model (rows).}
%         \label{fig:ovno-ranking-gap5}
%     \end{subfigure}
%     \vspace{-15pt}
%     \caption{Neural vs. baseline methods for beam search with width value set to 5 (SCIP oracle). (a) Win counts; (b) Log-likelihood gaps. Color: Darker green = stronger, darker red = weaker performance. Grey: Timeouts (30s).}
%     \label{fig:combined-gap5}
% \end{wrapfigure}


==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/algorithms/beam_search_algo.tex <==
\begin{wrapfigure}[20]{r}{0.5\textwidth} 
\vspace{-10pt} % tweak vertical space if needed
\begin{algorithm}[H]
\DontPrintSemicolon
\KwIn{PGM $\mathcal{M}$, Scoring Function $\mathcal{F}$, Evidence $\mathbf{E}$, Time Limit $tl$, Maximum Decisions $\mathcal{D}_{max}$, Beam Width $W$}
\KwOut{MPE Solution}
Initialize beam $B \gets [(0, \mathbf{E})]$ \; % (score, updated evidence)

\For{$d = 1$ to $\mathcal{D}_{max}$}{
    Initialize candidate list $C \gets []$\;
    \ForEach{$(s, E_{updated})$ in $B$}{
        \ForEach{variable-value pair $(X, x)$}{
            $E_{new} \gets E_{updated} \cup (X = x)$\;
            $s_{new} \gets \mathcal{F}(E_{new})$\;
            $(s_{new}, E_{new})$ to $C$\;
        }
    }
    $B \gets$ Sort $C$ by $s$ and retain top $W$ sequences\;
}

$(s_{best}, \mathbf{E_{best}}) \gets \text{TopCandidate}(B)$\;
$\text{rec} \gets \texttt{SolveMPE}(\mathcal{M}, \mathbf{E_{best}}, tl)$\;
\Return $\text{rec}$
\caption{Beam Search for Conditioning}\label{alg:beam_search}
\end{algorithm}
\vspace{-10pt} % tweak to control space below the figure
\end{wrapfigure}

==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/algorithms/data_collection.tex <==
\begin{wrapfigure}[28]{r}{0.55\textwidth} % r for right side, 0.55 width (adjust as needed)
\vspace{-12pt} % tweak vertical space if needed
\begin{algorithm}[H]
\DontPrintSemicolon

\KwIn{PGM $\mathcal{M}$, Query Ratio $qr$, Dataset Type $dt$, Max Depth $d_{max}$, Max Choices $c_{max}$}
\KwOut{Dataset $DB$}

\textbf{Function} \texttt{SolveMPE}($\mathcal{M}, \mathbf{E}, \mathbf{e}$): \\
\Indp
    Run MPE solver on $\mathcal{M}$ with $\mathbf{E} = \mathbf{e}$\;
    \Return $\{ \text{time}, \text{\#nodes}, \text{assign} \}$ \\
\Indm

\textbf{Function} \texttt{Sample}($\mathbf{S}, n$): \\
\Indp
    \Return Randomly selected $n$ elements from $\mathbf{S}$\;
\Indm

$\mathbf{X} = \mathbf{x} \leftarrow \text{Sample generated from } \mathcal{M}$ \;
$\mathbf{Q} \gets \texttt{Sample}(\mathcal{V}, qr \cdot |\mathcal{V}|)$ \; 
$\mathbf{E} \gets \mathcal{V} \setminus \mathbf{Q}$ \tr{define $\mathcal{V}$}\;
%$d \gets \texttt{Sample}(\{0, 1, \dots, d_{max}\}, 1)$  \;

%$\mathbf{Q_d} \gets \texttt{Sample}(\mathbf{Q}, d)$ \;
%$\mathbf{E} \gets \mathbf{E} \cup \mathbf{Q_d}, \quad \mathbf{Q} \gets \mathbf{Q} \setminus \mathbf{Q_d}$ \;

$\text{rec} \gets \texttt{SolveMPE}(\mathcal{M}, \mathbf{E}, \mathbf{x}_{\mathbf{E}})$ \;

\If{$dt = \text{ranking}$}{
    $\text{opt} \gets \text{rec}[\text{assign}]$ \;
    $\mathbf{C} \gets \texttt{Sample}(\mathbf{Q}, c_{max})$ \;
    
    \For{each $C \in \mathbf{C}$}{
        $c \gets \text{opt}[C]$ \;
        $\mathbf{E}^{'} \gets \mathbf{E}, \quad \mathbf{e}^{'} \gets \mathbf{e}$ \;
        $\mathbf{E}^{'} \gets \mathbf{E}^{'} \cup \{C\}, \quad \mathbf{e}^{'} \gets \mathbf{e}^{'} \cup \{c\}$\;
        $\text{rec} \gets \texttt{SolveMPE}(\mathcal{M}, \mathbf{E}^{'}, \mathbf{e}^{'})$
    }
}

\text Store in DB

\caption{Data Collection for Training Neural Network for Conditioning}\label{algo:dataset}
\end{algorithm}
\vspace{-10pt} % tweak to control space below the figure
\end{wrapfigure}

==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/fig_tex_files/decimation_daoopt.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/gap-vs-node.pdf}
    \caption{Greedy conditioning methods (AOBB oracle): Average solution gap (x-axis) versus \% node reduction (y-axis). Each subfigure denotes a fixed decision count.}
    \label{fig:daoopt-gap}
\end{figure*}

==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/fig_tex_files/decimation_scip.tex <==
\begin{wrapfigure}[47]{r}{0.275\linewidth}
    \vspace{-10pt} % Adjust as needed to align with surrounding text
    \centering
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figures/win-comparison.pdf}
        \caption{Wins vs. oracle by time limit for all methods (G: Graph, SB: Full Strong Branching, LO: \textsc{L2C-OPT}, LR: \textsc{L2C-Rank}).}
        \label{fig:win-comparison}
    \end{subfigure}
    \vspace{1em}
    \begin{subfigure}{\linewidth}
        \includegraphics[width=\linewidth]{figures/ovno-ranking-gap.pdf}
        \caption{\textsc{L2C-Rank} vs. oracle $\mathcal{LL}$ gap by $\mathcal{D}_{max}$ (cols) and graphical model (rows).}
        \label{fig:ovno-ranking-gap}
    \end{subfigure}
    \vspace{-15pt}
    \caption{Neural vs. baseline methods for greedy conditioning (SCIP oracle). (a) Win counts; (b) Log-likelihood gaps. Color: Darker green = stronger, darker red = weaker performance. Grey: Timeouts (30s).}
    \label{fig:combined-gap}
\end{wrapfigure}


==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/fig_tex_files/decimation_scip3.tex <==
\begin{figure}[htbp]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/supplement/win-comparison3.pdf}
    \label{fig:win-comparison3}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/supplement/win-comparison5.pdf}
    \label{fig:win-comparison5}
  \end{subfigure}
  \caption{Neural vs. baseline methods for beam search with width value set to 3 (SCIP oracle). (a) Win counts; (b) Log-likelihood gaps. Color: Darker green = stronger, darker red = weaker performance. Grey: Timeouts (30s).}
  \label{fig:combined-wins}
\end{figure}

\FloatBarrier

% \begin{wrapfigure}[47]{r}{0.275\linewidth}
%     \vspace{-10pt} % Adjust as needed to align with surrounding text
%     \centering
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/supplement/win-comparison3.pdf}
%         \caption{Wins vs. oracle by time limit for all methods (SB: Full Strong Branching, LO: \textsc{L2C-OPT}, LR: \textsc{L2C-Rank}).}
%         \label{fig:win-comparison3}
%     \end{subfigure}
%     \vspace{1em}
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/supplement/ovno-ranking-gap3.pdf}
%         \caption{\textsc{L2C-Rank} vs. oracle $\mathcal{LL}$ gap by $\mathcal{D}_{max}$ (cols) and graphical model (rows).}
%         \label{fig:ovno-ranking-gap3}
%     \end{subfigure}
%     \vspace{-15pt}
%     \caption{Neural vs. baseline methods for beam search with width value set to 3 (SCIP oracle). (a) Win counts; (b) Log-likelihood gaps. Color: Darker green = stronger, darker red = weaker performance. Grey: Timeouts (30s).}
%     \label{fig:combined-gap3}
% \end{wrapfigure}


==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/fig_tex_files/decimation_scip5.tex <==
\begin{figure}[htbp]
  \centering
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/supplement/ovno-ranking-gap3.pdf}
    \label{fig:ovno-with-ranking-gap3}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures/supplement/ovno-ranking-gap5.pdf}
    \label{fig:ovno-with-ranking-gap5}
  \end{subfigure}
  \caption{Neural vs. baseline methods for beam search with width value set to 3 (SCIP oracle). (a) Win counts; (b) Log-likelihood gaps. Color: Darker green = stronger, darker red = weaker performance. Grey: Timeouts (30s).}
  \label{fig:combined-ovno-with-ranking-gap}
\end{figure}

\FloatBarrier
% \begin{wrapfigure}[47]{r}{0.275\linewidth}
%     \vspace{-10pt} % Adjust as needed to align with surrounding text
%     \centering
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/supplement/win-comparison5.pdf}
%         \caption{Wins vs. oracle by time limit for all methods (G: Graph, SB: Full Strong Branching, LO: \textsc{L2C-OPT}, LR: \textsc{L2C-Rank}).}
%         \label{fig:win-comparison5}
%     \end{subfigure}
%     \vspace{1em}
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/supplement/ovno-ranking-gap5.pdf}
%         \caption{\textsc{L2C-Rank} vs. oracle $\mathcal{LL}$ gap by $\mathcal{D}_{max}$ (cols) and graphical model (rows).}
%         \label{fig:ovno-ranking-gap5}
%     \end{subfigure}
%     \vspace{-15pt}
%     \caption{Neural vs. baseline methods for beam search with width value set to 5 (SCIP oracle). (a) Win counts; (b) Log-likelihood gaps. Color: Darker green = stronger, darker red = weaker performance. Grey: Timeouts (30s).}
%     \label{fig:combined-gap5}
% \end{wrapfigure}


==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/fig_tex_files/results_variable_selection_heuristic.tex <==
% Results for our neural solver used as branching variable section strategy
\begin{wrapfigure}[22]{r}{0.275\linewidth}
    \vspace{-10pt} % Adjust as needed to align with surrounding text
    \centering
    \includegraphics[width=\linewidth]{figures/neural-search-gap.pdf}
    \caption{Heuristic comparison across datasets (rows) and time limits (columns); darker green/red indicates better/worse \textsc{L2C-Rank} performance.}
    \label{fig:ns-gap}
    % \vspace{-10pt} % Adjust as needed to align with surrounding text
\end{wrapfigure}


% \begin{wrapfigure}{r}{0.3\linewidth}
%     \centering
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/ovno-ranking-gap.pdf}
%         \caption{Gap for Decimation: Increasing decimation decisions increases the gap, demonstrating scalability of Decinet-Rank. X-axis marks columns for number of decisions taken as percentage of size of the query variables and Y-axis indicates rows for the particular graphical model. Larger negative gap indicated by darker green shade shows better performance in terms of the log-likelihood achieved.}
%         \label{fig:ovno-ranking-gap}
%     \end{subfigure}
%     \vspace{1em}
%     \begin{subfigure}{\linewidth}
%         \includegraphics[width=\linewidth]{figures/neural-search-gap.pdf}
%         \caption{Decinet-Rank vs. SCIP: Negative average gap indicates superior performance of our neural search heuristic over default SCIP across datasets plotted against the three timelimits. Darker shade of green indicates better performance. X-axis marks columns for the timelimit (in seconds) alloted to the oracle and Y-axis indicates rows for the particular graphical model.}
%         \label{fig:ns-gap}
%     \end{subfigure}
%     \caption{Performance of Decinet-Rank. (\textbf{Top})  Scalability with increasing decimation decisions. (\textbf{Bottom}) Comparison of Neural Search Heuristics with default SCIP.}
%     \label{fig:combined-gap}
% \end{wrapfigure}

==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/sections/1_intro.tex <==
\section{Introduction}\label{sec:intro}

Probabilistic Graphical Models (PGMs) \citep{koller2009probabilistic}, such as Bayesian Networks and Markov Networks, efficiently encode joint probability distributions over a large set of random variables, enabling structured reasoning under uncertainty. A fundamental inference task in these models is the Most Probable Explanation (MPE) query, where the goal is to find the most likely assignment of values to unobserved variables given observed evidence.

Answering MPE queries is computationally intractable in general due to their NP-hardness, and becomes particularly challenging as model complexity and scale increase. Classical exact methods—such as AND/OR search~\citep{AOBB, marinescu2010daoopt} and integer linear programming (ILP)~\citep{koller2009probabilistic}—guarantee optimality but are prohibitively expensive for large instances. Approximate methods offer scalability but often compromise on solution quality or consistency, especially in domains that demand high-precision inference.
% Although such solvers often support \textit{anytime inference}—providing the best solution found upon interruption—their performance frequently remains insufficient under stringent time constraints, limiting their applicability in real-time scenarios.

Conditioning on a variable subset\textemdash fixing variables to specific values\textemdash is a common strategy for improving the tractability of inference by simplifying the underlying problem structure. This reduction in complexity can significantly shrink the search space and improve solver performance. This principle underlies classical techniques like cutset conditioning \citep{pearl_dechter_cutset_conditioning} and recursive conditioning \citep{darwiche_recursive_2001}, as well as strong branching heuristics \citep{10.1007/s10107-023-01977-x, applegate} in ILP solvers. A related concept in statistical physics is \emph{decimation} \citep{Mezard2002-ej,SP-SAT,kroc_message-passing_2009,burjorjee_explaining_2012,10.5555/1835372}, which iteratively fixes high-impact variables to reduce the search space in message-passing algorithms such as Survey Propagation, progressively simplifying the problem instance. However, the effectiveness of these methods is highly sensitive to the choice and ordering of conditioned variables; poor decisions can lead to significant degradation in solution quality.

This leads to a fundamental question: \emph{which variables should be fixed, to which values, and in what order, to simplify inference while preserving the optimal solution?} Fixing variables incorrectly can irrevocably exclude the true optimal solution, whereas deferring all conditioning preserves completeness but forfeits the computational benefits of simplification. Ideally, conditioning decisions should be both \emph{safe}—i.e., aligned with optimal solutions—and \emph{useful}—i.e., significantly reduce computational effort.

In principle, access to the complete set of MPE solutions for a given instance would enable the identification of such beneficial assignments. For instance, if a variable assumes the same value across all optimal solutions, fixing it would preserve optimality and likely simplify the subsequent problem. In practice, however, enumerating all MPE solutions is infeasible \citep{NEURIPS2019_fc2e6a44}, and exhaustively evaluating the impact of every variable-value pair on solver performance is prohibitively expensive. Consequently, existing methods rely on handcrafted heuristics \citep{CSI-Poole, fridman2003mixed} or structure-based metrics \citep{kjaerulff1990triangulation} that often lack generalization.

In this work, we introduce \emph{learning to condition} (L2C), a \emph{data-driven} approach to rank variable-value assignments based on their utility for conditioning. The goal is to train a neural network to identify assignments that strike a balance between two objectives: preserving access to optimal solutions and simplifying the inference process. To achieve this, we train an attention-based neural network that assigns two scores to each variable-value assignment: an \emph{optimality score}, estimating the likelihood of the assignment's presence in an optimal solution, and a \emph{simplification score}, measuring the extent to which fixing the assignment reduces solver effort.

We obtain supervision for these scores via a scalable data generation pipeline. For each training instance, we solve the MPE query once using an oracle and treat the resulting solution as a proxy for the set of optimal solutions. Variable-value pairs present in the solution are labeled as positive examples for the optimality head. To supervise the simplification head, we fix individual variables to their optimal values, re-solve the query, and record solver statistics such as runtime and the number of explored nodes, providing a quantitative measure of the reduction in inference complexity.

A key insight of our method is that solution ambiguity modulates conditioning risk. If a variable takes the same value across all optimal solutions, fixing it is highly effective—but also risky if the estimate is incorrect, as it could eliminate the true MPE solution. Conversely, when a variable's values are more evenly distributed, conditioning poses less risk. Even if the model slightly misestimates the correct value, the solution space is more tolerant, and optimality may still be preserved. Our model implicitly learns to navigate this trade-off by generating soft scores that reflect both expected utility and uncertainty, shaped through diverse training examples.

At inference time, the model assigns scores to all variable-value pairs in the query set for the given instance and conditions on those with the highest scores. This strategy incrementally simplifies the problem while avoiding premature elimination of the optimal solution. Additionally, the learned model can also be integrated into branch-and-bound solvers as node and variable selection heuristics.

\vspace{0.5em}
\noindent\textbf{Contributions.} This paper introduces a neural network-based conditioning strategy for MPE inference in PGMs, with the following key contributions:

\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
\item We formalize \emph{learning to condition} (L2C) as a scoring problem over variable-value pairs that jointly optimizes for solution preservation and inference tractability.

\item We design a data-efficient supervision strategy that generates labels using oracle solutions and solver statistics, avoiding the need for exhaustive MPE enumeration.

\item We introduce an attention-based architecture that generalizes across instances and yields informative optimality and simplification scores.

\item We demonstrate that our method improves both inference efficiency and solution quality over classical heuristics across a range of benchmark PGMs.
\end{itemize}


Our results show that L2C enables scalable, learned conditioning decisions that adapt to instance structure, outperforming traditional heuristics in both speed and accuracy.


==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/sections/2_background.tex <==
\section{Background}
\label{background}

We assume, w.l.o.g., that all random variables are binary and take values in \( \{0,1\} \). Individual variables are denoted by uppercase letters (e.g., \( X \)), and their assignments by corresponding lowercase letters (e.g., \( x \)). Sets of variables are denoted by bold uppercase letters (e.g., \( \mathbf{X} \)), and assignments to those sets are written in bold lowercase (e.g., \( \mathbf{x} \)). Given a full assignment \( \mathbf{x} \) to a set \( \mathbf{X} \), and a subset \( \mathbf{Y} \subseteq \mathbf{X} \), we use \( \mathbf{x}_{\mathbf{Y}} \) to denote the projection of \( \mathbf{x} \) onto \( \mathbf{Y} \).

A \textbf{probabilistic graphical model} (PGM) \( \mathcal{M} = \langle \mathbf{X}, \mathbf{F}, G \rangle \) is defined over a set of variables \( \mathbf{X} \), a collection of log-potentials \( \mathbf{F} = \{ f_1, \dots, f_m \} \), and an undirected primal graph \( G = (\mathcal{V}, \mathcal{E}) \). Each log-potential \( f_i \in \mathbf{F} \) is defined over a subset \( \mathbf{S}(f_i) \subseteq \mathbf{X} \), known as its scope. The vertex set \( \mathcal{V} \) contains one node for each variable in \( \mathbf{X} \), and an edge \( (\mathcal{V}_a, \mathcal{V}_b) \in \mathcal{E} \) is added whenever \( X_a \) and \( X_b \) co-occur in the scope of some \( f_i \). The model defines the following joint probability distribution:
\[
P_{\mathcal{M}}(\mathbf{x}) \propto \exp\left( \sum_{f \in \mathbf{F}} f(\mathbf{x}_{\mathbf{S}(f)}) \right)
\]

We focus on the \textbf{most probable explanation (MPE)} task: given observed evidence variables \( \mathbf{E} \subset \mathbf{X} \) with assignment \( \mathbf{e} \), find the most likely assignment for query variables \( \mathbf{Q} = \mathbf{X} \setminus \mathbf{E} \). Formally, this is:
\[
\text{MPE}(\mathbf{Q}, \mathbf{e}) = \arg\max_{\mathbf{q}} P_{\mathcal{M}}(\mathbf{q} \mid \mathbf{e}) = \arg\max_{\mathbf{q}} \sum_{f \in \mathbf{F}} f((\mathbf{q}, \mathbf{e})_{\mathbf{S}(f)})
\]

This problem is NP-hard in general and remains intractable for numerous model families~\citep{cooper_1990_complexityprobabilistic, park&darwiche04, decamposNewComplexityResultsMAPBayesianNetworks, conaty17, peharz2015foundations}.

Exact MPE algorithms include bucket elimination~\citep{dechter99}, which uses variable elimination via local reparameterization, and Mixed Integer Programming (MIP) encodings solved with branch-and-bound solvers like SCIP~\citep{BolusaniEtal2024OO} that combine LP relaxations with systematic search. Such solvers are often anytime, providing progressively better solutions and bounds, with optimality certificates upon convergence. Nevertheless, for many real-world PGMs\textemdash particularly those with high treewidth\textemdash exact inference remains computationally infeasible. 


\textbf{Conditioning} is a classical strategy for simplifying inference by fixing a subset of variables. For MPE, assigning values $\mathbf{q}_d$ to a conditioning set $\mathbf{Q}_d \subseteq \mathbf{Q}$ reduces the problem to solving MPE for the remaining variables $\mathbf{Q}_0 = \mathbf{Q} \setminus \mathbf{Q}_d$ given evidence $\mathbf{e} \cup \mathbf{q}_d$. The resulting residual solution $\mathbf{q}_0^*$ and $\mathbf{q}_d$ form the complete MPE solution. Conditioning is fundamental to exact methods like cutset conditioning \cite{pearl_dechter_cutset_conditioning}, recursive conditioning \cite{darwiche_recursive_2001}, and search algorithms such as Branch and Bound (B\&B) and AND/OR Branch and Bound (AOBB) \cite{marinescu_2009_branch-and-boundsearch}. Conditioning also informs heuristic methods such as decimation strategies inspired by statistical physics~\citep{SP-SAT, kroc_message-passing_2009, Montanari2007SolvingCS, Cai-decimation-maxsat}.

\textbf{Branch and Bound (B\&B)} performs a depth-first or best-first search over a decision tree, recursively partitioning the assignment space and pruning subproblems using lower bounds from LP relaxations or mini-bucket elimination~\citep{MBApprox}; its efficiency hinges on branching heuristics and bound quality.  \textbf{AND/OR Branch and Bound (AOBB)}~\citep{marinescu_2009_branch-and-boundsearch} improves upon B\&B by exploiting graphical model structure through a \textit{pseudo tree} and an AND/OR search graph. This graph uses OR nodes for variable choices and AND nodes for decomposition points, enabling independent search on conditionally independent components formed by assignments. AOBB further avoids redundant computations by merging nodes with identical separator contexts. Consequently, AOBB can prune substantial portions of the search space, often achieving exponential savings over standard B\&B.%, especially for low-treewidth models.

Graph-based methods like Mini-Bucket Elimination~\citep{MBApprox} generate bounds (e.g., upper bounds for MPE) that accelerate B\&B and AOBB through earlier pruning. Variable and value ordering heuristics further enhance their effectiveness~\citep{siddiqi2008variable, marinescu2006dynamic, marinescu2003systematic}.

Recent efforts integrate learning into solver decisions. In MIP, \textit{full strong branching}~\citep{applegate, 10.1007/s10107-023-01977-x} uses one-step look-ahead for selecting branch variables that maximize bound improvement; neural networks trained via imitation learning can replicate this~\citep{Khalil, Gasse}. Other machine learning approaches include using SVMs to identify optimal decision variables~\citep{Yuan-ML-Problem-reduction} and NNs for effective node-selection strategies~\citep{Shen-PB-DFS}. Recent neural approaches to MPE inference have concentrated on optimizing relaxed likelihood objectives~\citep{arya_2024_networkapproximatorsa, arya2024_nn_mpe_nips, 2025sine}. While these methods eliminate the need for supervision, they provide no guarantees of optimality, as they rely on continuous relaxations of the MPE objective.

Our work advances \textit{conditioning-based simplification} by learning a scoring function that ranks variable-value assignments according to their utility in reducing inference complexity while preserving optimality. 


==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/sections/3_data_collection.tex <==
\subsection{Data collection}
\label{subsec:data}
We construct a dataset of MPE queries and solver outcomes to train the L2C model to score variable-value assignments based on two criteria: their consistency with optimal solutions and their ability to simplify inference when fixed. Because enumerating all optimal solutions or exhaustively evaluating all assignments is computationally infeasible, we collect targeted supervision using selective oracle queries under randomized input conditions.


 The full data collection procedure is described in Algorithm~\ref{algo:conditioning-data}. Given a probabilistic graphical model \( \mathcal{M} = \langle \mathbf{X}, \mathbf{F}, G \rangle \), we repeatedly sample full assignments \( \mathbf{x} \sim P_{\mathcal{M}} \) and randomly partition the variable set into disjoint subsets: a query set \( \mathbf{Q} \subset \mathbf{X} \) of size \( qr \cdot |\mathbf{X}| \), and an evidence set \( \mathbf{E} = \mathbf{X} \setminus \mathbf{Q} \). The evidence assignment \( \mathbf{e} \) is formed by projecting \( \mathbf{x} \) onto \( \mathbf{E} \), and an MPE solver is invoked to compute the optimal solution \( \mathbf{q}^* = \arg\max_{\mathbf{q}} P_{\mathcal{M}}(\mathbf{q} \mid \mathbf{e}) \). The resulting assignment, along with runtime and number of nodes explored, is stored as supervision.

\begin{wrapfigure}[24]{r}{0.45\textwidth}
\vspace{-15pt}
\begin{algorithm}[H]
\footnotesize
\DontPrintSemicolon

\KwIn{PGM \( \mathcal{M} = \langle \mathbf{X}, \mathbf{F}, G \rangle \), Query Ratio \( qr \), Max Conditions \( c_{\max} \), Budget $B$}
\KwOut{Dataset \( DB \)}

\textbf{Function} \texttt{SolveMPE}(\( \mathcal{M}, \mathbf{e}, B \)): \\
\Indp
    Run MPE solver on \( \mathcal{M} \) with evidence \( \mathbf{e} \) and time bound $B$\;
    \Return \( \text{rec} = \{ \text{assign}, \text{time}, \#\text{nodes} \} \) \;
\Indm

\vspace{3pt}

Initialize \( DB \gets \emptyset \) \;

\While{not enough samples in \( DB \)}{
    Sample \( \mathbf{x} \sim P_{\mathcal{M}} \) \;
    \( \mathbf{Q} \gets \text{random subset of } \mathbf{X} \text{ of size } qr  |\mathbf{X}| \) \;
    \( \mathbf{E} \gets \mathbf{X} \setminus \mathbf{Q} \) \;
    \( \mathbf{e} \gets \mathbf{x}_{\mathbf{E}} \) \;

    \( \text{rec} \gets \texttt{SolveMPE}(\mathcal{M}, \mathbf{e}) \) \;
    Store \( (\mathbf{e}, \text{rec}) \) in \( DB \) \;

    \( \mathbf{C} \gets \text{random subset of } \mathbf{Q} \text{ of size } c_{\max} \) \;

    \For{each \( C \in \mathbf{C} \)}{
        \For{each value \( c \in \{0, 1\} \)}{
            \( \mathbf{e}' \gets \mathbf{e} \cup \{C = c\} \) \;
            \( \text{rec}' \gets \texttt{SolveMPE}(\mathcal{M}, \mathbf{e}') \) \;
            Store \( (\mathbf{e}', \text{rec}') \) in \( DB \) \;
        }
    }
}

\Return \( DB \)
\caption{Data Collection for L2C with Conditioning Assignments}
\label{algo:conditioning-data}
\end{algorithm}
\vspace{-10pt}
\end{wrapfigure}To evaluate the impact of variable-value assignments on inference, we randomly sample a subset \( \mathbf{C} \subset \mathbf{Q} \) of size at most \( c_{\max} \), and for each \( C \in \mathbf{C} \), consider both binary assignments \( C = 0 \) and \( C = 1 \). For each assignment, we augment the evidence to form \( \mathbf{e}' = \mathbf{e} \cup \{C = c\} \), solve the resulting MPE query, and record solver statistics such as runtime, number of nodes explored, and objective value. These evaluations provide supervision for both the simplification and optimality scoring heads.

Evaluating all possible variable-value assignments for each instance is computationally prohibitive, especially for large models. To manage this cost, we introduce a sampling parameter \( c_{\max} \) that bounds the number of variables considered for conditioning per instance. This allows us to gather informative supervision while keeping the number of additional MPE queries tractable.  In practice, \( c_{\max} \) can be chosen based on the model size, the characteristics of the solver, and the available compute budget.

When the solver fails to return a result within the allocated time budget $B$, we log surrogate statistics such as LP-bound improvements or relaxed objective scores. Although these surrogates may be noisy, they increase coverage across instances and improve the generalization ability.% of the learned simplification scores.

%The value of \( c_{\max} \) controls a tradeoff between dataset richness and computational efficiency: higher values yield more training signals but incur greater solver overhead.

%To evaluate the impact of conditioning on inference, we randomly sample a subset \( \mathbf{C} \subset \mathbf{Q} \) of size at most \( c_{\max} \), and for each \( C \in \mathbf{C} \), evaluate both binary assignments \( C = 0 \) and \( C = 1 \). For each assignment, we augment the evidence to form \( \mathbf{e}' = \mathbf{e} \cup \{C = c\} \), solve the resulting conditioned MPE query, and record solver statistics such as runtime, number of nodes explored, and objective value. These records provide supervision for both simplification and optimality scoring. Because conditioned solves are computationally expensive, we limit their number per instance using the parameter \( c_{\max} \), which bounds the number of variables selected for evaluation. Additionally, when a conditioned query exceeds the solver’s time limit, we store surrogate statistics such as LP-bound improvements or relaxed objective values. While these surrogates may be noisy, they enable broader dataset coverage and improve the generalization and robustness of the learned simplification scores. In practice, \( c_{\max} \) can be selected based on the complexity of the underlying solver and the computational budget available for data generation.


%To evaluate simplification effects, we randomly sample a subset \( \mathbf{C} \subset \mathbf{Q} \) of size at most \( c_{\max} \), and for each \( C \in \mathbf{C} \), evaluate both binary assignments \( C = 0 \) and \( C = 1 \). For each such assignment, we augment the evidence to form \( \mathbf{e}' = \mathbf{e} \cup \{C = c\} \), solve the conditioned query, and record solver statistics. This yields supervision for both simplification and optimality scores. 

%Each unconditioned instance provides binary labels indicating whether a variable-value pair \( (Q_i = q) \) matches the oracle output \( \mathbf{q}^* \), serving as supervision for the optimality head. 

Each $\mathbf{e}$ and its corresponding optimal assignment $\mathbf{q}^*$ (if returned by the MPE solver) in $DB$ serves as supervision for the optimality head. For simplification, we convert the collected solver statistics into a ranking distribution over a small set of candidate variables \( \mathbf{C} \subset \mathbf{Q} \). For each candidate \( C \in \mathbf{C} \), we define:
$
p_C \propto \frac{1}{t_C}$
where \( t_C \) is a composite scalar derived from multiple solver statistics recorded for the query conditioned on \( C = c \), including runtime, number of search nodes explored, and objective value. These quantities are combined linearly to reflect the overall simplification utility of the assignment. The resulting distribution is normalized using a softmax over inverse scores, assigning higher probabilities to variable-value assignments that are more effective at reducing inference cost.

Thus the resulting dataset contains both exact and surrogate supervision, allowing the model to learn to balance optimality preservation with inference simplification across a range of graphical model instances.

%The resulting dataset captures both forms of supervision: exact oracle-labeled assignments for unmodified queries, which indicate consistency with optimal MPE solutions, and solver statistics—exact or surrogate—associated with fixing variable-value pairs under modified evidence, which reflect simplification utility. Because solver calls are computationally intensive, simplification statistics are recorded only for a subset of query variables, and surrogate metrics are used when timeouts occur. Despite this partial supervision, the dataset spans a diverse range of problem instances and conditioning scenarios. This enables the model to jointly learn two complementary objectives: preserving the correctness of the final solution and reducing the computational effort required to obtain it. As a result, the model acquires a robust internal notion of which variable-value assignments are both reliable and useful for inference-time decision making.

%The resulting dataset includes both exact supervision for optimality—based on oracle solutions—and approximate supervision for simplification—based on solver statistics for a subset of variable-value assignments. This partial yet diverse supervision enables the model to learn to balance solution accuracy with inference efficiency across a wide range of problem instances.




%For simplification, we convert the collected solver statistics into a ranking distribution over the candidates \( \mathbf{C} \). Specifically, we define:
% $
% p_C \propto \frac{1}{t_C}
% $, 
%where \( t_C \) is a composite scalar derived from multiple solver statistics for the query conditioned on \( C = c \), such as runtime, number of search nodes explored, and objective value. These quantities are combined linearly to reflect the overall simplification utility of each assignment. This normalized inverse-score distribution (softmax) assigns higher probability to assignments that simplify inference more effectively.


% Each unconditioned instance provides binary labels indicating whether a variable-value pair \( (Q_i = q) \) matches the oracle output \( \mathbf{q}^* \), serving as supervision for the optimality head. For simplification, we convert the collected solver statistics into a ranking distribution over the candidates \( \mathbf{C} \). Specifically, we define:
% \[
% p_C = \frac{1/t_C}{\sum_{C' \in \mathbf{C}} 1/t_{C'}}
% \]

%where \( t_C \) is the runtime for solving the query conditioned on \( C = c \). This softmax over inverse runtimes assigns higher probability to assignments that reduce inference time. While runtime is our default statistic, the ranking distribution can also incorporate other metrics such as objective value or number of nodes explored.

%Because conditioned solves are expensive, ranking supervision is generated only for a sampled subset of variable-value pairs. For instances where the oracle exceeds a time limit, we fall back to surrogate signals such as LP-bound improvements or relaxed objectives. These weaker signals enable broader dataset coverage and improve the robustness of simplification score learning.

% Thus the resulting dataset contains both exact and surrogate supervision, allowing the model to learn to balance optimality preservation with inference simplification across a range of graphical model instances.



% Training a model to score variable-value assignments requires supervision that captures both their impact on preserving MPE solution quality and their ability to simplify inference when fixed. Since exhaustive evaluation of all assignments or optimal solutions is computationally prohibitive, we generate partial yet informative supervision by selectively querying an MPE oracle and observing solver behavior under targeted input modifications.

% Given a probabilistic graphical model \( \mathcal{M} = \langle \mathbf{X}, \mathbf{F}, G \rangle \), we begin by sampling a complete assignment \( \mathbf{x} \sim P_{\mathcal{M}} \), and partition the variable set into disjoint evidence and query subsets \( \mathbf{E} \subset \mathbf{X} \), \( \mathbf{Q} = \mathbf{X} \setminus \mathbf{E} \). After projecting \( \mathbf{x} \) to \( \mathbf{E} \) to form evidence \( \mathbf{e} \), we use an MPE oracle to find the optimal query assignment \( \mathbf{q}^* \) (for \( \arg\max_{\mathbf{q}} P_{\mathcal{M}}(\mathbf{q} \mid \mathbf{e}) \)), recording \( \mathbf{q}^* \), solver runtime, and explored nodes. Candidate query assignments $(Q_i = q)$ are then labeled based on consistency with \( \mathbf{q}^* \), providing supervision for optimality.

% To estimate the effect of conditioning, we select a candidate variable subset \( \mathbf{C} \subset \mathbf{Q} \) (where \( |\mathbf{C}| \leq c_{\max} \)). For each \( C \in \mathbf{C} \), we fix its value according to \( \mathbf{q}^* \) and re-solve the MPE query using augmented evidence \( \mathbf{E}' = \mathbf{E} \cup \{C\} \). We record solver statistics (such as runtime, node count, objective value) for each conditioned query. These statistics serve as proxies for the inference simplification utility of fixing each variable.

% Instead of directly predicting solver statistics, we convert them into instance-specific rankings over the sampled assignments. Assignments achieving greater simplification\textemdash e.g., lower runtime or fewer nodes explored during branch-and-bound search\textemdash receive higher ranks. These rankings serve as supervision for training the network’s simplification head, enabling it to learn to prioritize assignments that effectively reduce inference cost. Sections~\ref{subsec:architecture} and~\ref{subsec:loss} detail the ranking procedure and loss formulation.

% For scalability, we limit conditioned queries per instance and apply oracle timeouts. If the MPE oracle exceeds its time budget, we use surrogate indicators like relaxed objective values or LP-bound progress. While less precise, these surrogates facilitate broader and more diverse data collection. We incorporate both exact and surrogate supervision during training to enhance model generalization and robustness. 


==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/sections/3_method.tex <==
\section{Learning to Condition (L2C)}
\label{sec:method}

We propose a neural approach for ranking variable-value assignments based on their utility in simplifying MPE inference while preserving optimality. This task, which we call \textbf{Learning to Condition (L2C)}, balances two goals: minimizing inference cost and avoiding exclusion of optimal solutions. Our model learns two scores per assignment: one measuring consistency with optimal solutions and another estimating simplification benefit. These data-driven scores guide the selection of high-confidence assignments and can also be used to steer node selection in B\&B solvers.
Next, we describe the L2C pipeline, including data generation, neural architecture, training objectives, ranking mechanism, and integration with inference procedures.

\input{sections/3_data_collection}

\subsection{Neural network architecture}
\label{subsec:architecture}

For a partially observed MPE instance (evidence \( \mathbf{E} \subset \mathbf{X} \) with assignment \( \mathbf{e} \), query variables \( \mathbf{Q} = \mathbf{X} \setminus \mathbf{E} \)), our model (Figure~\ref{fig:architecture}) scores variable-value pairs on their potential for MPE optimality preservation and inference cost reduction. Each pair \( (X_i = x_i) \) is represented by an embedding vector \citep{Mikolov2013EfficientEO}. For binary variables, an embedding table of size \( 2 \times |\mathbf{X}| \) provides distinct embeddings for each variable's possible values. An additional embedding indicates variable status (observed/evidence or unobserved/query), enabling support for arbitrary evidence-query partitions.

For each unobserved variable $Q_i \in \mathbf{Q}$, its two value assignment embeddings query a multi-head attention module \citep{Attention} using evidence variable embeddings as keys and values, contextualizing each candidate assignment relative to the instance and enabling the model to learn associations between evidence and promising assignments. The output contextualized embeddings, concatenated with their original counterparts, pass through a shared encoder (comprising fully connected layers with ReLU activations, residual connections \citep{Residual}, and dropout \citep{srivastava_waypreventneural_2014}). This encoder produces a representation for each variable-value pair, which is then passed to two separate prediction heads.

The \emph{optimality head}, a two-layer MLP with a sigmoid output, estimates an assignment's likelihood of inclusion in the MPE solution. Trained with binary cross-entropy loss against oracle-derived labels, this head learns a relaxed optimality proxy, capturing generalizable patterns across problem instances.

A separate \emph{simplification head}, also a two-layer MLP, outputs unnormalized scores for candidate assignments. These scores, after softmax normalization, are trained via a list-ranking cross-entropy loss \cite{Cao-l2r}, using targets derived from solver statistics (Section~\ref{subsec:data}) like runtime, search depth, or relaxed objectives. By predicting relative utility instead of absolute complexity reduction, this head produces scores that generalize well and exhibit noise robustness.

Our architecture exhibits permutation invariance to variable ordering and supports arbitrary evidence-query partitions, promoting generalization. Cross-attention facilitates query-specific evidence conditioning, while the dual-head design jointly optimizes solution quality and inference efficiency. This yields a flexible scoring function adept at guiding conditioning during inference.


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/Architecture.pdf}
    \caption{Attention-based architecture for scoring variable-value pairs by their utility in simplifying MPE inference while preserving optimality.}
    \label{fig:architecture}
\end{figure}


\subsection{Loss functions}
\label{subsec:loss}

We train our model using a multi-task objective \citep{caruana1997multitask} that combines two losses: a binary classification loss for predicting whether a variable-value pair is part of an optimal MPE solution, and a list-ranking loss that encourages the model to prioritize assignments that simplify inference. These respectively supervise the network's optimality and simplification heads.

\paragraph{Optimality loss.} For each query variable \( Q_i \in \mathbf{Q} \) and its possible values \( q_i \in \{0,1\} \), the optimality head predicts \( \hat{y}_i^{(q)} \in [0,1] \), the probability that assignment \( Q_i = q \) is in the oracle MPE solution, where \( y_i^{(q)} \in \{0,1\} \) is the true label. The binary cross-entropy loss is applied independently per pair:
\[
\mathcal{L}_{\text{opt}} = - \sum_{Q_i \in \mathbf{Q}} \sum_{q \in \{0,1\}} \left( y_i^{(q)} \log \hat{y}_i^{(q)} + (1 - y_i^{(q)}) \log (1 - \hat{y}_i^{(q)}) \right)
\]
This formulation supports supervision with multiple optimal assignments, enabling the model to learn from all optimal solutions for a given instance.

\paragraph{Simplification ranking loss.} For each instance, the training dataset contains solver statistics for a subset of query variables \( \mathbf{C} \subset \mathbf{Q} \), obtained during data collection as described in Section~\ref{subsec:data}. For each \( C \in \mathbf{C} \), we construct a target probability distribution \( p_C \) that reflects the simplification utility of fixing \( C = c \), based on a combination of solver statistics such as runtime, number of nodes explored, and objective value. The simplification head generates scores for all variable-value pairs in \( \mathbf{Q} \), which are normalized via softmax into a predicted distribution \( \hat{p}_C \). We then compute a list-ranking cross-entropy loss \cite{Cao-l2r}:
\[
\mathcal{L}_{\text{rank}} = - \sum_{C \in \mathbf{C}} p_C \log \hat{p}_C
\]
This loss encourages the model to prioritize assignments that lead to greater reductions in inference cost. Since supervision is available only for a subset of \( \mathbf{Q} \), we apply a binary mask to restrict the loss computation to the subset \( \mathbf{C} \) for which solver statistics were recorded during training. This ensures that only observed variable-value pairs influence parameter updates, while predictions for the rest of \( \mathbf{Q} \) remain unconstrained.

\begin{wrapfigure}[23]{r}{0.45\textwidth}
\vspace{-15pt}
\begin{algorithm}[H]
\footnotesize
\DontPrintSemicolon
\KwIn{PGM \( \mathcal{M} \), Scoring function \( \mathcal{F} \), Initial evidence \( \mathbf{E} \), Time limit \( tl \), Max depth \( \mathcal{D}_{\max} \), Beam width \( W \)}
\KwOut{Approximate MPE solution}

Init. beam \( B \gets \{(0, \mathbf{E})\} \) \texttt{//(score,evid)}

\For{\( d = 1 \) to \( \mathcal{D}_{\max} \)}{
    Initialize candidate list \( C \gets \emptyset \)\;
    \ForEach{\( (s, \mathbf{E}_{\text{partial}}) \in B \)}{
        Identify query variables \( \mathbf{Q}_{\text{rem}} = \mathbf{X} \setminus \mathbf{E}_{\text{partial}} \)\;
        \ForEach{unfixed \( Q_i \in \mathbf{Q}_{\text{rem}} \)}{
            \ForEach{value \( q_i \in \{0, 1\} \)}{
                Let \( \mathbf{E}' \gets \mathbf{E}_{\text{partial}} \cup \{Q_i = q_i\} \)\;
                Let \( s' \gets \mathcal{F}(\mathbf{E}') \)\;
                Add \( (s', \mathbf{E}') \) to \( C \)\;
            }
        }
    }
    Sort \( C \) in descending order by score \( s' \)\;
    Prune \( C \) to retain top \( W \) elements\;
    \( B \gets C \)\;
}

Let \( (s^*, \mathbf{E}^*) \gets \textsc{TopCandidate}(B) \)\;
Run \( \mathbf{q}^* \gets \texttt{SolveMPE}(\mathcal{M}, \mathbf{E}^*, tl) \)\;
\Return \( \mathbf{q}^* \)
\caption{Beam Search for L2C}
\label{alg:beam_search}
\end{algorithm}
\end{wrapfigure}

\paragraph{Joint objective and masking.} The total loss combines these components as a weighted sum:
\[
\mathcal{L} = \lambda_{\text{opt}} \cdot \mathcal{L}_{\text{opt}} + \lambda_{\text{rank}} \cdot \mathcal{L}_{\text{rank}}
\]
Here, \( \lambda_{\text{opt}} \) and \( \lambda_{\text{rank}} \) balance the objectives' relative importance. We train using both exact and surrogate datasets. If supervision is available for only one head (optimality or ranking), we apply its loss and mask the other, preventing gradient updates from missing targets. This joint objective allows the model to balance accuracy with inference efficiency by leveraging both exact and approximate supervision.


\subsection{Inference-time strategies}
\label{subsec:inference}

At inference time, the model guides variable-value assignment decisions that simplify the MPE problem before the solver is invoked. Given a probabilistic graphical model \( \mathcal{M} = (\mathbf{X}, \mathcal{F}) \), an initial evidence set \( \mathbf{E} \subset \mathbf{X} \), and assignment \( \mathbf{e} \), the model takes the current evidence as input and produces scores for each remaining query variable-value pair \( (Q_i = q_i) \), where \( Q_i \in \mathcal{V} \setminus \mathbf{E} \) and \( q_i \in \{0,1\} \).

The \textit{optimality head} outputs confidence \( \hat{y}_i^{(q)} \in [0,1] \) for an assignment's MPE consistency; the \textit{simplification head} provides a score \( s_i^{(q)} \in \mathbb{R} \) for its inference simplification utility. These scores are combined to select conditioning assignments via two strategies:

\paragraph{Greedy conditioning.} This strategy iteratively filters assignments by an optimality threshold \( \tau \), selects the one with the highest simplification score among confident candidates, and adds it to evidence. This repeats for a fixed number of steps or until no confident options remain, before passing the simplified MPE query to a solver.

\input{fig_tex_files/decimation_scip}


\paragraph{Beam search.} To explore multiple conditioning sequences, beam search (Algorithm~\ref{alg:beam_search}) maintains \( W \) partial assignment sequences. At each step \( d \leq \mathcal{D}_{\max} \), sequences are expanded with assignments scored as in greedy conditioning. The best final sequence provides evidence \( \mathbf{E}^* \) for the MPE solver.

\paragraph{Final solution.} Let \( \mathbf{E}^* \) denote the final evidence set selected by either strategy. The residual MPE query is defined over \( \mathbf{Q}_{\text{residual}} = \mathcal{V} \setminus \mathbf{E}^* \). We call an MPE solver (exact or anytime) to compute:
\[
\mathbf{q}_{\text{residual}}^* = \arg\max_{\mathbf{q}} P_{\mathcal{M}}(\mathbf{q} \mid \mathbf{e}^*)
\]

and return the complete solution \( \mathbf{q}^* = \mathbf{q}_{\text{residual}}^* \cup \mathbf{e}^* \).


This framework uses learned assignments to restructure the MPE problem, reducing solver complexity while preserving correctness and enabling time-bounded inference.


\paragraph{NN-Guided branch-and-bound search}
\label{subsec:nn_for_bnb}

Our neural model also enhances branch-and-bound (B\&B) solvers. It guides branching by selecting variables predicted to simplify the subproblem (using scores akin to greedy conditioning) and uses optimality head predictions to tighten lower bounds. These actions accelerate B\&B convergence while maintaining optimality guarantees.

Learning to Condition (L2C) transforms the traditionally static variable selection problem into a learned, instance-specific decision process. Compatible with both exact and approximate solvers, L2C generalizes across problem instances and enables principled trade-offs between solution quality and computational cost. We next empirically evaluate its performance across a diverse set of benchmarks and graphical models.


==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/sections/4_experiments.tex <==
\section{Experiments}\label{expts}

In this section, we evaluate our neural strategies, \textsc{L2C-Opt} (using only the optimality head for scoring) and \textsc{L2C-Rank} (using the scoring procedure from Section~\ref{subsec:inference}). We benchmark these strategies for two tasks: (1) against standard conditioning heuristics, and (2) as branching and node selection methods within B\&B solvers. We
begin by describing our experimental framework, including the PGMs, baseline methods, evaluation metrics, and NN architecture.


\subsection{Graphical models}
We evaluated our method and baselines on 14 high-treewidth binary probabilistic graphical models (PGMs) from UAI inference competitions \citep{elidan_2010_2010, UAICompetition2022}, featuring 90 to 1444 variables and up to 1444 factors. Using Gibbs sampling \citep{koller2009probabilistic}, we generated 12{,}000 training, 1{,}000 test, and 1{,}000 validation examples per model.  All MPE instances used 75\% of the PGM's variables as query variables. We construct the supervised dataset following the procedure outlined in Section~\ref{subsec:data}. During data generation, QR is set to 0.75  and $c_{\text{max}}$ is set to 10\% of the total number of variables in each PGM.

\subsection{Experimental setup and methods}


The neural networks in \textsc{L2C-Opt}  and \textsc{L2C-Rank} use 256-dimensional embeddings, two multi-head attention layers, and 15 skip-connection blocks. Dense layers have 512 units with 0.1 dropout \citep{srivastava_waypreventneural_2014} and ReLU activations. We trained the models using Adam \citep{kingma_stochasticoptimization_2017} with a learning rate of $8 \times 10^{-4}$, an exponential decay rate of 0.97, a batch size of 128, and early stopping after 5 stagnant epochs (maximum 50 epochs). All models were implemented in PyTorch \citep{paszke2019pytorch} and executed on an NVIDIA A40 GPU. The supplementary material provides further hyper-parameter details.

\input{fig_tex_files/decimation_daoopt}

\paragraph{Baseline methods:}
We compare our approach with two heuristic methods: The \textbf{graph-based heuristic} \citep{siddiqi2008variable, marinescu2006dynamic, marinescu2003systematic} prioritizes variables by degree, selecting them in descending order after removing evidence nodes. This max-degree strategy assigns each variable its most likely value, estimated via Gibbs Sampling \citep{koller2009probabilistic, pmlr-vR2-kask99a} over the PGM. The \textbf{full strong branching heuristic} \citep{applegate}, a classical technique for enhancing branch-and-bound efficiency, formulates the MPE query as an ILP \citep{koller2009probabilistic}. It then scores variable-value pairs by their impact on search space pruning.

\paragraph{Oracle:}
We use two oracles on unconditioned queries and as final solvers post-conditioning: the SCIP solver \citep{BolusaniEtal2024OO}, and the AND/OR Branch and Bound (AOBB) solver (per \citet{marinescu_2009_branch-and-boundsearch} and implemented by \citet{marinescu2010daoopt}). MPE queries are encoded as Integer Linear Programs (ILPs) \citep{koller2009probabilistic} for SCIP, which applies its branch-and-bound algorithm subject to a 60-second time limit per query.

\paragraph{Evaluation criteria:}
The competing approaches were evaluated based on two criteria: log-likelihood scores and runtime. The log-likelihood scores, calculated as \( \ln p_\mathcal{M}(\mathbf{e}, \mathbf{q}) \), assesses the quality of the solution in terms of optimality. The runtime measures the efficiency of the conditioning process by indicating how quickly each method solves the problem.

\subsection{Empirical evaluations} 

\subsubsection{Greedy conditioning}

We evaluate our methods and baselines as scoring functions ($\mathcal{F}$) in a greedy conditioning framework (Section~\ref{subsec:inference}), selecting up to 25\% of query variables.\footnote{To ensure a fair comparison, as the max-degree baseline supports only a beam size of 1, we use greedy conditioning for neural and strong branching methods. Supplementary material provides beam search results.} For each PGM, we test 12 configurations: four conditioning depths (5\%, 10\%, 15\%, 25\% of query variables) combined with three oracle time budgets (10s, 30s, 60s). Post-conditioning, SCIP attempts to solve the residual problem within the allotted budget.

Figure~\ref{fig:win-comparison} (heatmap) quantifies for each conditioning strategy the number of the 12 configurations where it enabled the SCIP oracle to achieve a higher average log-likelihood ($\mathcal{LL}$) score than solving the original, non-conditioned query. The oracle's time budget was identical for both conditioned and non-conditioned queries.

The results (Figure~\ref{fig:win-comparison}) show that both \textsc{L2C-Opt} (LO) and \textsc{L2C-Rank} (LR) consistently enhance oracle performance over direct solving of the original query. \textsc{L2C-Rank} performs best, frequently surpassing the non-conditioned oracle across all 12 configurations. Conversely, full strong branching (SB) and the graph-based heuristic (G) only occasionally improve $\mathcal{LL}$ scores.

Figure~\ref{fig:ovno-ranking-gap} presents the average percentage $\mathcal{LL}$ gap:
$
\frac{1}{N} \sum_{i=1}^{N} (\mathcal{LL}_{S}^{(i)} - \mathcal{LL}_{D}^{(i)})/(|\mathcal{LL}_{S}^{(i)}|) \times 100,
$
where $\mathcal{LL}_{S}^{(i)}$ and $\mathcal{LL}_{D}^{(i)}$ are the oracle's log-likelihoods for instance $i$ without and with conditioning by \textsc{L2C-Rank}, respectively. Rows denote PGMs, and columns indicate conditioning depth (percentage of query variables conditioned). The oracle's time budget is fixed at 30s for both approaches.


Predominantly negative (green) values in Figure~\ref{fig:ovno-ranking-gap} indicate that \textsc{L2C-Rank} conditioning helps the oracle find superior solutions within the 30s budget. The gap becomes increasingly negative with more conditioning decisions (i.e., greater conditioning depth), demonstrating our method's scalability. This improvement occurs because conditioning simplifies the query by instantiating additional variables, thus presenting an easier query to the oracle.

\paragraph{Assisting AOBB via conditioning:}

We also evaluated our neural heuristic with the AND/OR Branch and Bound (AOBB) solver \citep{marinescu2010daoopt} as an alternative oracle. 

Figure~\ref{fig:daoopt-gap} plots the percentage reduction in AOBB's processed node count (y-axis, proxy for effort reduction) against the average $\mathcal{LL}$ gap from the exact MPE solution (x-axis).\footnote{Node and $\mathcal{LL}$ gap reductions for AOBB are relative to its unconditioned execution. AOBB's internal preprocessing and heuristics often enable it to solve MPE queries within the time limit; thus, a reduced node count with a near-zero $\mathcal{LL}$ gap signifies simplified inference without quality loss.} Points near the y-axis indicate high solution quality with reduced effort; greater x-values imply more quality degradation.

\input{fig_tex_files/results_variable_selection_heuristic}

Our conditioning strategies, as shown in Figure~\ref{fig:daoopt-gap}, yield near-optimal solutions while substantially reducing AOBB's processed node count. In contrast, traditional baselines exhibit larger solution gaps with increased conditioning depth due to increasingly suboptimal decisions. Our methods consistently maintain high solution quality (most points near the y-axis) and more effectively accelerate AOBB by shrinking the search space, particularly with deeper conditioning.

Consequently, L2C enables efficient resolution of queries that are otherwise challenging for the oracle, especially for large-treewidth models, frequently yielding substantially better solutions under identical time constraints.

\subsubsection{NN-Guided branch-and-bound search}
We also employ our neural network outputs to guide branch-and-bound search, using them as branching rules \citep{Gasse} and node selection heuristics \citep{Shen-PB-DFS}, following the methodology detailed in Section~\ref{subsec:nn_for_bnb}.

Figure~\ref{fig:ns-gap} compares our neural-guided heuristics against SCIP’s default strategies \citep{BolusaniEtal2024OO, Achterberg2012, Archterberg-Hybrid-Branching, Wallace2009}, showing the average $\mathcal{LL}$ gap (defined previously) over three time limits and all datasets. The predominantly green cells, particularly dark green ones, in the heatmap signify that our neural heuristics often outperform SCIP's defaults. Furthermore, the few red cells underscore that our approach generally matches or surpasses SCIP's default heuristic performance and delivers better solutions within identical time budgets.

\paragraph{Summary:} Our comprehensive experiments validate the consistent superiority of L2C. As a conditioning strategy, it empowers SCIP to achieve better solutions within time limits, especially for intractable problems, and allows AOBB to preserve solution quality while drastically reducing search effort (node exploration). Furthermore, employing our neural scores as branching and node selection heuristics enhances SCIP's solution quality under the same time constraints. Collectively, these results affirm our method's effectiveness both as a conditioning strategy—improving solution quality and efficiency—and as an effective heuristic guiding branch-and-bound solvers.


==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/sections/5_conclusion.tex <==
\section{Conclusion and future work}

We introduced \textit{Learning to Condition} (L2C), a neural approach leveraging solver search traces to accelerate Most Probable Explanation (MPE) inference in Probabilistic Graphical Models (PGMs). L2C learns to identify variable assignments that effectively balance inference simplification with optimality preservation, superseding handcrafted heuristics. It serves either as a pre-processor simplifying problems for exact solvers or as an internal policy guiding branching and variable selection within search algorithms. Evaluations on high-treewidth models show L2C substantially curtails the search space, achieving solution quality comparable or superior to baselines and thus providing a more efficient path to MPE solutions.

Future work will target L2C's current limitations in scalability, solver signal quality, and the scope of learned guidance. We will adapt L2C for larger models (millions of variables and factors), necessitating efficient large-scale data collection. Richer solver signals (e.g., branch-and-cut decisions) will be integrated for more aggressive pruning, improving upon current signal usage. Finally, learned variable orderings will be explored for novel neural bounding strategies, extending guidance beyond conditioning to further boost inference performance.

==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/sections/6_supplement_content.tex <==
\section{Description of the probabilistic graphical models} \label{dataset}

Table~\ref{tab:datasets} summarizes the networks used in our experiments, listing the number of variables and factors in each. The experiments were conducted on high-treewidth probabilistic graphical models (PGMs) of varying sizes, with the number of variables ranging from 90 to 1440 and factor counts covering a similar range.

\begin{table}[ht!]
    \centering
    \caption{Summary of networks used in our experiments, including the number of variables and factors for each.}
    \label{tab:datasets}
    \begin{tabular}{|c|c|c|}
    \hline
    Network           & Number of Factors & Number of Variables \\ 
    \hline
    BN 12             & 90      & 90           \\ 
    BN 9              & 105     & 105          \\ 
    BN 13             & 125     & 125          \\ 
    Grid 20           & 1200    & 400          \\ 
    BN 65             & 440     & 440          \\ 
    BN 59             & 540     & 540          \\ 
    BN 53             & 561     & 561          \\ 
    BN 49             & 661     & 661          \\ 
    BN 61             & 667     & 667          \\
    BN 45             & 880     & 880          \\
    Promedas 68       & 1022    & 1022         \\
    Promedas 60       & 1076    & 1076         \\
    BN 30             & 1156    & 1156         \\
    BN 32             & 1440    & 1440         \\
    \hline
    \end{tabular}
\end{table}

\section{Hyperparameter details}

We used a consistent set of hyperparameters across all networks in our experiments. From the initial dataset of 14{,}000 samples, we allocated 13{,}000 for training and 1{,}000 for testing. The training set was further split into 12{,}000 samples for training and 1{,}000 for validation.

The neural networks in \textsc{L2C-Opt} and \textsc{L2C-Rank} use 256-dimensional embeddings, two multi-head attention layers, and 15 skip-connection blocks. Each dense layer contains 512 units and applies a dropout rate of 0.1. The neural networks were trained using the Adam optimizer with a learning rate of $8 \times 10^{-4}$ and an exponential decay factor of $0.97$. Training was performed for up to $50$ epochs with a batch size of $128$, employing early stopping if validation performance did not improve for 5 consecutive epochs. After training, we evaluated the model on 1{,}000 MPE queries with a query ratio of $0.75$, defined as the fraction of variables in the query set.

Hyperparameters were selected via 5-fold cross-validation. In particular, the weighting parameters $\lambda_{opt}$ and $\lambda_{rank}$ were critical for balancing the preservation of optimal solutions with inference efficiency. We searched over $\lambda_{opt} \in \{0.3, 0.35, 0.4, 0.45, 0.5\}$ and set $\lambda_{rank} = 1 - \lambda_{opt}$.

\section{Comparing conditioning methods by per-decision time}

Table~\ref{tab:dt-comp} reports the average time required to make a single conditioning decision across all networks. The decision times for \textsc{L2C-Opt} and \textsc{L2C-Rank} remain stable across network sizes, demonstrating their scalability. In contrast, the graph-based heuristic shows increasing latency with network size, while strong branching is significantly slower and often impractical. We imposed a 30-second timeout per decision, under which strong branching failed to return results on the largest networks, BN 30 and BN 32.

\begin{table}[ht]
    \centering
    \caption{Average decision time (in seconds). Dashed cells indicate instances where the 30-second timeout was reached.}
    \label{tab:dt-comp}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|l|l|c|c|c|c|}
    \toprule
    Methods & \textsc{L2C-Opt} & \textsc{L2C-Rank} & Graph & Strong Branching \\
    Network Name &  &  &  &  \\
    \midrule
    \textbf{BN 12} & 0.001 ± 0.000 & 0.002 ± 0.001 & 0.001 ± 0.001 & 2.215 ± 0.161 \\
    \textbf{BN 9} & 0.003 ± 0.002 & 0.006 ± 0.004 & 0.007 ± 0.003 & 1.256 ± 0.115 \\
    \textbf{BN 13} & 0.001 ± 0.001 & 0.002 ± 0.001 & 0.022 ± 0.020 & 2.787 ± 0.114 \\
    \textbf{Grid 20} & 0.006 ± 0.004 & 0.011 ± 0.004 & 0.107 ± 0.062 & 7.325 ± 0.117 \\
    \textbf{BN 65} & 0.005 ± 0.005 & 0.008 ± 0.005 & 0.086 ± 0.053 & 5.871 ± 0.320 \\
    \textbf{BN 59} & 0.005 ± 0.004 & 0.009 ± 0.005 & 0.097 ± 0.057 & 10.993 ± 1.683 \\
    \textbf{BN 49} & 0.007 ± 0.005 & 0.011 ± 0.004 & 0.100 ± 0.059 & 19.713 ± 3.417 \\
    \textbf{BN 53} & 0.005 ± 0.004 & 0.009 ± 0.005 & 0.095 ± 0.056 & 9.106 ± 0.993 \\
    \textbf{BN 61} & 0.009 ± 0.004 & 0.013 ± 0.004 & 0.103 ± 0.063 & 20.896 ± 3.038 \\
    \textbf{BN 45} & 0.011 ± 0.005 & 0.014 ± 0.003 & 0.088 ± 0.050 & 8.675 ± 0.733 \\
    \textbf{Promedas 68} & 0.013 ± 0.004 & 0.016 ± 0.003 & 0.085 ± 0.051 & 4.279 ± 0.118 \\
    \textbf{Promedas 60} & 0.015 ± 0.002 & 0.015 ± 0.002 & 0.089 ± 0.052 & 5.432 ± 0.270 \\
    \textbf{BN 30} & 0.018 ± 0.002 & 0.018 ± 0.002 & 0.098 ± 0.058 & $-$ \\
    \textbf{BN 32} & 0.023 ± 0.005 & 0.025 ± 0.009 & 0.102 ± 0.060 & $-$ \\
    \bottomrule
    \end{tabular}
    }
\end{table}

\section{Greedy conditioning performance using SCIP as oracle}

In this section, we analyze the conditioning performance of all methods under varying oracle time budgets and numbers of greedy conditioning decisions when SCIP solver \citep{BolusaniEtal2024OO} is used as the oracle. For each method and network, we report the average percentage gap in log-likelihood. The y-axis in Figures~\ref{fig:PR_BN_12} to \ref{fig:PR_BN_32} shows the average percentage gap in log-likelihood scores, computed as:

\begin{equation} \label{eq:2}
   \text{avg.}~ \% ~\text{gap} =  \frac{1}{N} \sum_{i=1}^{N} \frac{(\mathcal{LL}_{S}^{(i)} - \mathcal{LL}_{D}^{(i)})}{|\mathcal{LL}_{S}^{(i)}|} \times 100
\end{equation}

where $\mathcal{LL}_{S}^{(i)}$ denotes the log-likelihood score of the oracle before conditioning, and $\mathcal{LL}_{D}^{(i)}$ denotes the score after conditioning for instance $i$. Thus, negative values indicate that conditioning improves solution quality, while positive values indicate a decline in performance. The x-axis represents the number of conditioning decisions, and each subfigure corresponds to a distinct oracle time budget.

As shown in the figures, our neural network-based strategies, \textsc{L2C-Opt} and \textsc{L2C-Rank}, consistently improve the oracle performance after conditioning, as evidenced by negative percentage gaps. In contrast, the \textbf{graph-based heuristic} and the \textbf{full strong branching heuristic} lead to improvements in only a small fraction of instances. Since these baselines do not produce optimal decisions, their performance generally worsens with increasing oracle time budgets, resulting in larger positive average gaps. This degradation becomes more pronounced as the number of conditioning decisions increases. In comparison, our approaches yield increasingly negative average gaps with more decisions, indicating consistent performance gains.

\input{fig_tex_files/supp-scip-timelimit-expts}

% \section{Decision time comparison for greedy conditioning}

% Table~\ref{tab:dt-comp} reports the time required to make a single decision during greedy conditioning across all networks. The decision times for \textsc{L2C-Opt} and \textsc{L2C-Rank} remain stable regardless of network size, demonstrating their scalability. In contrast, the graph-based heuristic exhibits increased decision times as network size grows. The strong branching heuristic is particularly inefficient, often requiring substantial time per decision. We imposed a 30-second time limit per conditioning decision, under which strong branching timed out on the largest networks, BN 30 and BN 32.

\section{Conditioning performance for beam search-based conditioning}

\subsection{Using SCIP as oracle}
We now present detailed results comparing the performance of various conditioning strategies when used in beam search, using the SCIP solver as the oracle. Each bar represents the average log-likelihood gap (computed using equation~\ref{eq:2}) before and after conditioning, aggregated over conditioning depths of 5\%, 10\%, 15\%, and 25\% of the query variables, and averaged across all MPE queries solved using the oracle. Each subfigure corresponds to a specific oracle time budget.

Our neural strategies, \textsc{L2C-Opt} and \textsc{L2C-Rank}, consistently outperform the \textbf{full strong branching heuristic} in improving oracle performance, as evidenced by the negative average percentage gap. As the beam width increases, the performance of our methods either improves or remains consistent. In contrast, the strong branching heuristic often fails to return a decision within the 30-second time limit on larger networks and wider beams. As a result, the corresponding bars are omitted in the plots. 

We omit results for the \textbf{graph-based heuristic}, as it only supports a beam width of 1 and is therefore not applicable in this setting.

\input{fig_tex_files/supp-beam-width-expts}

\subsection{Using AOBB as oracle}

In this section, we evaluate the performance of beam search-based conditioning with AOBB (per \citet{marinescu_2009_branch-and-boundsearch} and implemented by \citet{marinescu2010daoopt}) as the oracle, using beam widths of 3 and 5, as shown in Figures~\ref{fig:aobb3} and \ref{fig:aobb5}, respectively. Each figure plots the average solution gap against the percentage reduction in the number of search nodes across 1,000 MPE queries over all networks, with each point representing one network. The solution gap is computed using Equation~\ref{eq:2}, while node reduction is calculated using the same formula with log-likelihood scores replaced by node counts before and after conditioning.

Our methods, \textsc{L2C-Opt} and \textsc{L2C-Rank}, consistently yield lower solution gaps—indicating better preservation of optimal solutions—and higher node reductions, reflecting improved search efficiency. In contrast, the full strong branching heuristic frequently fails to preserve solution quality, as indicated by its larger gaps, and produces fewer data points due to timeouts exceeding the 30-second limit per decision.

As before, we omit results for the \textbf{graph-based heuristic}, as it supports only a beam width of 1 and is therefore not applicable in this setting.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/supplement/gap-vs-node-bw3.pdf}
    \caption{Beam search-based conditioning with AOBB as the oracle using a beam width of 3. Each subfigure corresponds to a fixed number of conditioning decisions. The x-axis indicates the average solution gap (lower is better), and the y-axis indicates the percentage reduction in node count (higher is better). Each point represents a single network.}

    \label{fig:aobb3}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/supplement/gap-vs-node-bw5.pdf}
    \caption{Beam search-based conditioning with AOBB as the oracle using a beam width of 5. Each subfigure corresponds to a fixed number of conditioning decisions. The x-axis indicates the average solution gap (lower is better), and the y-axis indicates the percentage reduction in node count (higher is better). Each point represents a single network.}
    \label{fig:aobb5}
\end{figure}

\section{Incorporating L2C scores as branching and node selection heuristics in branch-and-bound}

In this section, we compare our trained neural networks—used as branching rules~\citep{Gasse} and node selection heuristics~\citep{Shen-PB-DFS} within the SCIP framework—with SCIP’s default heuristics~\citep{BolusaniEtal2024OO, Achterberg2012, Archterberg-Hybrid-Branching}. We evaluate performance based on the average percentage gap in log-likelihood (LL) scores between our methods, \textsc{L2C-Opt} and \textsc{L2C-Rank}, and SCIP’s default strategies on the same set of MPE queries. The gap is computed as:

\begin{equation} \label{eq:3}
\frac{1}{N} \sum_{i=1}^{N} \frac{\mathcal{LL}_{S}^{(i)} - \mathcal{LL}_{N}^{(i)}}{|\mathcal{LL}_{S}^{(i)}|} \times 100
\end{equation}

where $\mathcal{LL}_{S}^{(i)}$ denotes the log-likelihood score achieved by SCIP's default heuristics, and $\mathcal{LL}_{N}^{(i)}$ denotes the score obtained using our \textsc{L2C} methods on the $i$-th instance. Negative values indicate that our methods perform better; positive values indicate superior performance by SCIP’s default heuristics.

As shown in Figures~\ref{fig:NS_BN_12} to \ref{fig:NS_BN_32}, the percentage gap is typically negative, demonstrating that our methods consistently yield higher log-likelihood scores than SCIP within the same time budget. This indicates that for time-constrained settings, \textsc{L2C-Opt} and \textsc{L2C-Rank} can find higher-quality solutions more efficiently than SCIP’s default branching and node selection strategies. Overall, our learned heuristics not only produce better decisions but also execute faster than the state-of-the-art methods implemented in SCIP.

\input{fig_tex_files/supp-neural-search}

==> hrqdcwdxyptsrfcgrssxkmmhcxftmcpb/title.tex <==
Learning to Condition: A Neural Heuristic \\ for Scalable MPE Inference
